Asynchronous Training of Word Embeddings for Large Text Corpora

Word embeddings are a powerful approach for analyzing language and have been widely popular in numerous tasks in information retrieval and text mining. Training embeddings over huge corpora is computationally expensive because the input is typically sequentially processed and parameters are synchronously updated. Distributed architectures for asynchronous training that have been proposed either focus on scaling vocabulary sizes and dimensionality or suffer from expensive synchronization latencies. In this paper, we propose a scalable approach to train word embeddings by partitioning the input space instead in order to scale to massive text corpora while not sacrificing the performance of the embeddings. Our training procedure does not involve any parameter synchronization except a final sub-model merge phase that typically executes in a few minutes. Our distributed training scales seamlessly to large corpus sizes and we get comparable and sometimes even up to 45% performance improvement in a variety of NLP benchmarks using models trained by our distributed procedure which requires $1/10$ of the time taken by the baseline approach. Finally we also show that we are robust to missing words in sub-models and are able to effectively reconstruct word representations.

==> eval-benchmarks.tex <==
\subsection{Evaluation Benchmarks}
\label{sec:benchmarks}
\begin{table}[ht!]
\centering
% this just makes the table bigger, maybe use tabularx which supports full textwidth tables
%\resizebox{\linewidth}{!}{
\begin{tabular}{llrr}
\hline
Benchmark & Task& \#unique & \#tests or\\
name&Type&words&  \#clusters\\
\hline
\men& Similarity& 751& 3000\\
\rg& Similarity&48& 65\\
\rw& Similarity& 2951& 2034\\
\ws& Similarity& 437& 353\\
\ap& Categorization& 402 & 21\\
\battig& Categorization& 4393 & 56\\
\google& Analogy& 905& 19558\\
\semeval& Analogy& 3224& 2531\\
\hline
\end{tabular}
%}
\caption{Benchmarks statistics.}
\label{tab:benchmarks}
\end{table}
In order to evaluate the performance of merged models, we used a subset of benchmarks suggested in \cite{jastrzebski2017evaluate}. Specifically, we select benchmarks to evaluate \emph{similarity, categorization and analogy}. In the following we will briefly introduce the  benchmarks used in this work (also summarized in Table~\ref{tab:benchmarks}).

\subsubsection{Similarity Benchmarks}
Similarity benchmarks contain pairs of words and a real-valued number (corresponding to each pair) denoting similarity between the words as judged by human assessors. The trained model is  used to predict similarity scores for each pair. Spearman's rank order correlation (Spearman's $\rho$) is then used to measure the correlation between the model predictions and ground truth. We evaluate on the following similarity benchmarks.
\begin{itemize}
% [leftmargin=0cm,itemindent=.4cm,labelwidth=\itemindent,labelsep=0cm,align=left]
	\item \textbf{\rg}: \rg is provided by Rubenstein and Goodenough in \cite{RG65Rubenstein1965contextual}. This dataset contains 65 pairs of word where each pair is associated with a similarity score on the scale of 0-4.

% 	\item \textbf{MTurk}: Produced by Radinsky et al. In \cite{MTurkRadinsky2011word}, Radinsky et al. leverage the Amazon's Mechanical Turk platform to assign for each pair of words a relevance score. Over 280 words pairs was evaluated and each pair of word was evaluated by 10 people on a scale of 1-5.

	\item \textbf{\rw}: \rw represents the Stanford Rare Word Similarity Dataset by Luong et al. from \cite{RWLuong-etal:conll13:morpho}. Words are divided into several frequency intervals. We consider 2034 pairs of words with low frequency (rare words) assessed on a scale of semantic similarity from 0 to 10 by humans.

%Those with frequency less than 5 were considered as junk words. Only the English words with non-zero number of synsets in WordNet were selected.



	\item \textbf{\men}: First referenced in \cite{MENBruni2014multimodal}, the \men dataset annotations were generated using Mechanical Turk. For each pair of words a similarity score on a scale of 0-50 is computed based on human judgments.
    %In this dataset the similarities and relatedness are not separated considered. In the evaluation the entire \emph{MEN} dataset is used.

\item \textbf{\ws}: The \ws ~\cite{WS353Finkelstein2001placing} benchmark contains $353$ word pairs, each associated with an average of $13$ to $16$ human
judgments on a scale of $0$ to $10$.

%The \emph{WS353} is split into two parts, referenced as \emph{WS353R}, where \emph{R} stands for \emph{Relevance}, and \emph{WS353S}, where \emph{S} stands for \emph{Similarity}.

% \item \textbf{SimLex999}: The dataset \cite{SimLex999Hill2015simlex} is announced by Hill et al. indicate the real similarity instead of relatedness or associations. Only those words refers to analogous objects are considered similar, instead of words acting the similar roles in the sentences.
\end{itemize}
% The first 4 datasets doesn't distinguish words relatedness with similarity, while the \emph{WS353} does the explicit separation and \emph{SimLex999} evaluates similarity between words only.
% \todo{Word2vec model is only applicable for similarity defined on affinity.}


% \begin{table*}[ht!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccc}
% \hline
% Approach & AP & Battig & MEN & RG65 & RW & WS353 & Google & SemEval2012\_2\\
% \hline
% \texttt{Partition(1/10,10)} & 0.582 & 0.420 & 0.719 & 0.725 & 0.232 & 0.596 & 0.615 & 0.162\\
% % \hline
% \texttt{Random(1/10,10)} & \textbf{0.604} & \textbf{0.435} & \textbf{0.740} & \textbf{0.757} & 0.209 & \textbf{0.637} & 0.654 & \textbf{0.188}\\
% \hline

% \texttt{Partition(1/100,100) } & 0.505 & 0.358 & 0.622 & 0.723 & 0.203 & 0.516 & 0.467 & 0.129\\
% % \hline
% \texttt{Random(1/100,100)} & 0.517 & 0.381 & 0.644 & 0.746 & 0.257 & 0.542 & 0.487 & 0.138\\
% \hline
% \texttt{Baseline} & 0.595 & 0.434 & 0.736 & 0.757 & \textbf{0.299} & 0.611 & \textbf{0.661} & 0.181\\
% \hline
% \end{tabular}
% }
% \caption{Comparison between \texttt{Random(.,.)} and \texttt{Partition} sampling approaches at different granularities. PCA is used as the merging method.}
% \label{tab:sampling-comp}
% \end{table*}



\subsubsection{Categorization Benchmarks}
%Categorization benchmarks cluster the words in categories.
Categorization benchmarks provide a predefined set of categories and the corresponding word assignments. For example, the words \texttt{audi, bmw} and \texttt{ford} belong to the category \texttt{car}.
%the words from one dataset are given in different files, that words belong to the same category are in one identical file. The task is to determine if the word vectors in the embedded space can be clustered into the ground truth categories.
The task is to determine if the trained word embeddings cluster into the ground truth categories. The goodness is measured by calculating the \emph{purity score} -- the number of words clustered in the correct category divided by the total number of words in the ground truth. We used the following benchmarks in our experiments:
\begin{itemize}
\item \textbf{\ap}: The benchmark from Almuhareb and Poesio \cite{almuhareb2005concept} chooses words which cluster naturally in English. The dataset consists of 402 words divided into 21 categories.

%ach cluster is combined with words with low/medium/high frequency, and low/medium/high ambiguous words.


%Categorization tests from Almuhareb et al. \cite{almuhareb2005concept} considers three factors to balance the dataset, class type, term frequency and ambiguity. They chose words which forms cluster naturally in English, each cluster is combined with words with low/medium/high frequency, and low/medium/high ambiguous words.
% \item \textbf{BLESS}: A categorical dataset introduced by Baroni et al. \cite{baroni2011we}
\item \textbf{\battig}: This benchmark was introduced by Battig et al. \cite{battig1969category}. It consists of 5321 words divided into 56 categories.
\end{itemize}

\subsubsection{Analogy Benchmarks}
Analogy tasks evaluate arithmetic operations in a word embedding space. Given three words $A$, $B$ and $C$, the task is to find a word $D$ such that $D$ is related to $C$ in the same way that $B$ is to $A$. For example, given \texttt{Paris} is the capital of \texttt{France}, can we find the correct word (\texttt{Germany}) that fulfills this relationship for \texttt{Berlin}? From the trained word embeddings, $\mathbf{D}$ corresponds to the word with highest cosine similarity to the vector $\mathbf{B}-\mathbf{A}+\mathbf{C}$ (where $\mathbf{A,B,C,D}$ are vector representations of the words). The metric reported here is the \emph{accuracy} of prediction. 
The benchmarks that we used are:
\begin{itemize}
\item \textbf{\google}: Introduced by Mikolov et al. in \cite{mikolov2013distributed}, it contains both word and phrase analogy tests but we used only the 19,558 word analogy tests in our experiments.
% \item \textbf{MSR}: The test set of Microsoft's RNN for NLP project. At first the most frequent comparative adjectives, plural nouns, possessive nouns and base form of verbs 100 each are selected. The analogy tests questions are generated from these selected words systematically. This test focuses mainly on the syntactical instead of semantical analogies between words.
%\todo{What is 'A will typically B' , is something missing ?}
\item \textbf{\semeval}: \semeval represents the SemEval-2012 Task 2 and was first presented in \cite{jurgens2012semeval}. This benchmark has a fixed set of relationship types. For instance ``$A$ is the goal of $B$'' or ``an $A$ will typically $B$''. It consists of 10,014 questions divided into 10 relationship classes.

%It not only contains relevant word pairs but also a real number, which indicates the strength and the 'direction' of the relation, positive numbers stands for the relationship between the test pairs is the same with the given standard and vice versa. 
\end{itemize}
In the next section we provide implementation details for the models created using our approach and the baseline.



==> extra-tables.tex <==
We further evaluate the asynchronously trained embeddings in a retrieval task. We employ a variant of the Neural Translation Language Model~\cite{zuccon} as the retrieval model in which we incorporate the embeddings. The query likelihood for this retrieval model is computed as follows:

\begin{equation}
P(q|d) = \Pi_{q_i \in q} P_{ntm} (q_i|d)
\end{equation}

\begin{equation}
P_{ntm}(q_i|d) = \Pi_{w \in d} P(q_i|w) P(w|d)
\end{equation}

where w is a unigram found in the document.

\begin{equation}
P(q_i|w) = \frac{\delta(q_i, w)}{\sum_{w' \in V} \delta(w,w')}
\end{equation}

Here $\delta$ represents the cosine similarity between the embeddings of the operand unigrams. This value depends on the embeddings used in the retrieval model. For tractability reasons, we restrict $\sum_{w' \in V} \delta(w,w')$ to the neighborhood (n=500) of $w'$.

$P(w|d)$ is computed using a standard maximum likelihood estimator. 

The test collection used in our experiments is 100 topics (50-150) from the TREC web adhoc retrieval track and the Clueweb09B document collection. Clueweb09B is the english subset of the Clueweb09 collection with over 50 million web pages. We removed all documents with a spam score of 70 or below using the Waterloo spam scorer. The proposed retrieval model was applied to the top 1000 documents (ranked by query likelihood using unigram language models with dirichlet smoothing, $\mu = 2000$ ).

%
% embedding	map@100	p@5	p@10
% base_line.pkl-0.0.run	0.0055	0.0306	0.0316
% partitioning_100_pca.pkl-0.0.run	0.0055	0.0469	0.0418
% partitioning_10_pca.pkl-0.0.run	0.0074	0.049	0.049
% sampling_100_pca_dim_500.pkl-0.0.run	0.0063	0.049	0.0388
% sampling_10_pca_dim_500.pkl-0.0.run	0.0061	0.0367	0.0418
%

% this table will be used for retrieval results
\begin{table*}[ht!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
Approach & MAP\_100 & P\_5 & P\_10 \\
\hline
\texttt{Random(1/10,10)} + Concat & 0.595 & 0.429 & \textbf{0.742} \\
% \hline
\texttt{Random(1/10,10)} + LRA & 0.560 & 0.327 & 0.685 \\
% \hline
\texttt{Random(1/10,10)} + PCA & \textbf{0.604} & \textbf{0.435} & 0.740 \\
\hline
\texttt{Random(1/100,100)} + Concat & \textbf{0.525} & 0.377 & 0.643 \\
\texttt{Random(1/100,100)} + LRA & -- & -- & --\\
% \hline
\texttt{Random(1/100,100)} + PCA & 0.517 & \textbf{0.381} & \textbf{0.644} \\
% \hline
\hline
\texttt{Baseline} & 0.595 & 0.434 & 0.736 \\
\hline
\end{tabular}
}
%----------------------------------------


\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccc}
\hline
name & AP & Battig & MEN & RG65 & RW & WS353 & Google & SemEval2012\_2\\
\hline
partition\_pca & 0.582 & 0.420 & 0.719 & 0.725 & \textbf{0.232} & 0.596 & 0.615 & 0.162\\
\hline
sampling\_pca & \textbf{0.604} & \textbf{0.435} & \textbf{0.740} & \textbf{0.757} & 0.209 & \textbf{0.637} & \textbf{0.654} & \textbf{0.188}\\
\hline
baseline & 0.595 & 0.434 & 0.736 & 0.757 & 0.299 & 0.611 & 0.661 & 0.181\\
\hline
\end{tabular}
}
\caption{Results comparison between sampling and partitioning by 1/10 sub-copora}
\label{tab:eval_1/10p}
\end{table}

\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccc}
\hline
name & AP & Battig & MEN & RG65 & RW & WS353 & Google & SemEval2012\_2\\
\hline
partition\_pca & 0.505 & 0.358 & 0.622 & 0.723 & 0.203 & 0.516 & 0.467 & 0.129\\
\hline
sampling\_pca & \textbf{0.517} & \textbf{0.381} & \textbf{0.644} & \textbf{0.746} & \textbf{0.257} & \textbf{0.542} & \textbf{0.487} & \textbf{0.138}\\
\hline
baseline & 0.595 & 0.434 & 0.736 & 0.757 & 0.299 & 0.611 & 0.661 & 0.181\\
\hline
\end{tabular}
}
\caption{Results comparison between sampling and partitioning by 1/100 sub-copora}
\label{tab:eval_1/100p}
\end{table}


\begin{table}[hb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccc}
\hline
name & AP & Battig & MEN & RG65 & RW & WS353 & Google & SemEval2012\_2\\
\hline
concat & 0.595 & 0.429 & \textbf{0.742} & 0.765 & 0.268 & 0.611 & 0.645 & 0.187\\
\hline
lra+vadd & 0.560 & 0.327 & 0.685 & \textbf{0.785} & 0.264 & 0.606 & \textbf{0.661} & 0.158\\
\hline
pca & \textbf{0.604} & \textbf{0.435} & 0.740 & 0.757 & 0.209 & \textbf{0.637} & 0.654 & \textbf{0.188}\\
\hline
baseline & 0.595 & 0.434 & 0.736 & 0.757 & 0.299 & 0.611 & 0.661 & 0.181\\
\hline
name & AP & Battig & MEN & RG65 & RW & WS353 & Google & SemEval2012\_2\\
\hline
concat & \textbf{0.525} & 0.377 & 0.643 & \textbf{0.746} & \textbf{0.257} & \textbf{0.542} & \textbf{0.487} & \textbf{0.138}\\
\hline
pca & 0.517 & \textbf{0.381} & \textbf{0.644} & \textbf{0.746} & \textbf{0.257} & \textbf{0.542} & \textbf{0.487} & \textbf{0.138}\\
\hline
baseline & 0.595 & 0.434 & 0.736 & 0.757 & 0.299 & 0.611 & 0.661 & 0.181\\
\hline
\end{tabular}
}
\caption{Evaluation results for merging  sub-corpora}
\label{tab:eval_1/100s}
\end{table}





==> intro.tex <==
\section{Introduction}

%Word embeddings are a powerful approach for analyzing language (Bengio et al., 2006; Mikolov et al., 2013a,b; Pennington et al., 2014). A word embedding method discovers distributed representations which capture the semantic similarity between the words and reflect a variety of other linguistic regularities (Rumelhart et al., 1986; Bengio et al., 2006; Mikolov et al., 2013c). 

%Fitted word embeddings can help us understand the structure of language and are useful for downstream tasks based on text.
%These distributive models for word representations in the form of word embeddings have been widely popular in numerous tasks in Natural Language Processing (NLP), Text mining and Information Retrieval (IR). 

Word embeddings, abstractly put, are low-dimensional, continuous and dense representations of words in a semantic vector space. These distributive models for word representations have been widely popular in numerous tasks in Natural Language Processing (NLP), Text mining and Information Retrieval (IR).  
%As a special and popular approach of distributed word representation, word embedding is broadly applied in several tasks in Neural Language Processing (NLP) as a De facto standard practice. 
Specific application in NLP include tasks such as syntactic parsing \cite{socher2013parsing}, sentiment analysis \cite{socher2013recursive}, machine translation \cite{cho2014learning}, image annotation \cite{weston2011wsabie} and in shallow or deep architectures \cite{goldberg2016primer}. In IR, they are typically used in query modeling~\cite{zamani2016queryLM}, document representations~\cite{zamani2016estimating} and in the  construction of neural models for ranking~\cite{mitra2017neural,mitra2017introduction,desm16}. 

Typically, such word representations are learned in an unsupervised manner from large text corpora -- traditionally by matrix factorization approaches~\cite{li2015word} and more recently by employing neural networks~\cite{mikolov2013distributed,mikolov2013linguistic}. We focus on the latter approach for training word embeddings since they've been shown to scale well to larger corpora. In what follows, when we refer to word embeddings we always refer to the representations trained using a neural network. 
\todo{Corrections to be made in the following paragraph : original word2vec model uses Asynchronous SGD so serializibility in SGD cannot be stated as a problem. We too use negative sampling, the differences with ~\cite{ji2016parallelizing} need to eb clarified}
A key problem, despite the scalable nature of training word representations is the fact that stochastic gradient descent (SGD) is employed for weight update. First, SGD is inherently sequential because of the dependency of $i+1$-th iteration of calculation on the result of $i$-th iteration and they might potentially try to update the same word representations. Each iteration must potentially wait for the update from the previous iteration to complete. Second, the cost of model update at each iteration is a function of the underlying number of parameters which is $O(V)$ where $V$ is the vocabulary size of the text corpus. This leads to high training times for large corpora even with the use of optimizations to \emph{negative sampling}~\cite{stergiou2017distributed,ji2016parallelizing}, sub-sampling and vocabulary pruning~\cite{mikolov2013distributed}. Approaches towards scaling training for word embeddings using SGNS (Skip-gram model with negative sampling) are based on careful model updates on a shared model by optimizing negative sampling~\cite{ji2016parallelizing}, vertically partitioning the vocabulary~\cite{ordentlich2016network,stergiou2017distributed} and sometimes allowing for lock-free updates~\cite{recht2011hogwild}. 

%These learnt representations from samples of inputs are then considered as later merged into a single model in the spirit of ensembles. Motived by this we ponder on the broad research question:

We however take a different yet simple approach inspired by recent works in combining embeddings from disparate sources~\cite{garten2015combining,muromagi2017linear,goikoetxea2016single}, i.e., we construct models on \emph{samples of the input} rather than the entire dataset. These learnt representations from samples of inputs are then systematically merged into a single model in the spirit of ensembles. In essence we ponder the broader research question:
\todo{rather than stating this as question, I will rewrite it as our discovery.}
\emph{Can we learn word representations on larger corpora by asynchronously learning word representations from samples of the original document collection ?}

Now this has two major advantages. First, models can be \emph{asynchronously trained} on each of the samples and hence the overall training time can be reduced by parallelization. To this extent training can be easily leveraged by highly scalable parallel data processing platforms. 
Secondly, these partial models or sub-models obtained from the first phase should be combined effectively to provide representations. To this effect,in this paper we dwell on two specific research questions :


% Secondly, ensembles over the input can be combined to potentially provide better representations.
% We hence explore the idea that if models can be trained in a parallel manner on samples of a large input collection and combined later in a reasonable way we could leverage distributed infrastructures like Map-Reduce to train word representations on large text corpora. Towards this, we pose the following research questions:

\begin{itemize}
	\item \textbf{RQ I : } How do we sample from large input text collections for building partial models or sub-models ?
    
    \item \textbf{RQ II : } How do we combine partial models or sub-models ?
\end{itemize}


%  In order to train a representative word representation model, the size of its corpus has to be very large and takes quite long time to training trough. 
% Moreover, the training process of a lot modern distributed word representations leverage stochastic gradient descent (SGD) to converge to local minimum, which is considered to be non-scalable because of the dependency of $i+1$-th iteration of calculation on the result of $i$-th iteration. 
In answering the first research question, we find that sentence-wise random sampling (with replacement) of the input corpora preserves word distributions as well as word-context distributions (for large enough samples). This allows us to build sub-models without deviating much from the representational capacity. \todo{What do we mean by representational capacity here ? I usually relate it to number of dimensions used.} More importantly, we show that such sampling can be parallelized easily and consequently sub-models can be trained in parallel. 
\todo{sampling approaches that do not share same input across training epochs : need to describe what is good or bad about that. at present it is stated as a statement which is difficult for the reviewer to relate as this work is the first of its kind to sue that.}
Moreover, for obtaining robust models we propose sampling approaches that do not share the same input across training epochs. 

% In order to train a well-performing word representation in scalable way, we in this paper propose several approaches. The basic scheme of our approaches are the same, we first divide the corpus with sub-sampling into several corporal fragments, then training sub-models independently on each fragment.

After the sub-models are created(in parallel), we propose merging approaches to combine these, possibly sparse, models into a single unified representation by learning  and  combining them using dimensionality reduction based approaches like PCA and LRA. 
We observe that models based on samples of 10\% of input perform better than models trained on 1\% input collections in terms of effectiveness in all benchmarks. Specifically, we see that random sampling on 10\% is better than partitioning for the NLP benchmarks while there is no perceivable difference between random sampling and partitioning in the IR benchmarks. Secondly, we surprisingly see than 10\% samples sometimes outperform the baseline approaches and we attribute this reason to the ensemble nature of the sub-models. Third, we investigated multiple merging approaches and conclude that PCA over the trained submodels provides the best efficiency effectiveness trade-off and is robust across multiple tasks. Finally, as expected, we observe $10\times$ improvement in training times with our sampling approaches using a distributed implementation with competitive or often better benchmark performance.


% This process is highly adequate for a Map-Reduce framework and can be used to shorten the training time of a well-performing word embedding model.

% The basic idea of word embedding is mapping every word within a vocabulary extracted from a set of documents (corpus) to vector in an vector space. The embedded vectors present some simple but useful algebraic structure \cite{arora2016linear}, \cite{mikolov2013distributed}, which implies underlying semantic relationship between the words in the corpus. Assuming the language we focus on is generated from a distribution depending on some lateral variables, the learning process of a word representation is then to estimate the 'real' distribution as well as the lateral variables, based on the corpus, which can be treated as samples from the global real world language. It is according to the week law of big number, that as amount of samples increases, the expectation of estimated lateral variables converges to the 'real' lateral variables in probability. That is why large corpora are needed for training the word representations. Details on word representation models will be introduced later on.


% The popular word embedding algorithm word2vec algorithm relies on the Stochastic Gradient Descent (SGD) for optimization on large scale corpus \cite{mikolov2013distributed}. The SGD process, however, is represented as follows:
% \begin{equation}\label{eq:sgd}
% w^{(t)}=w^{(t-1)}-\eta_t\psi_{i_t}(w^{(t-1)})\text{,}
% \end{equation}
% where $w$ are the latent variable to find, $t$ represents iteration times, $i$ represents that within this round of descent, $\psi$ is calculated based on a sample from ${1,\ldots,n}$ and $\psi$ it self represents the loss function to minimize. According to the equation \ref{eq:sgd}, the $t$-th round calculation can be only calculated based on the result of $(t-1)$-th round. This not only causes the slow rate of convergence, but also restricts the possibility of scaling up the learning process in parallel. Several approaches on scaling the word embedding has been done by either reducing the variance of SGD \cite{recht2011hogwild} \cite{keuper2015asynchronous}, or optimizing the framework of word2vec program \cite{ordentlich2016network} \cite{ji2016parallelizing} \cite{eickhoff2016efficient}, or even presenting an incremental calculation framework \cite{kaji2017incremental}. We will later briefly introduce them and discuss their pro and cons, as well as the advantages also with the deficiency of our approach.



% \subsection{Contributions and Results}

In sum, in this paper we make the following contributions :

\begin{itemize}
\item We propose asynchronous methods for training word embedding models (using SGNS) on large input text corpora based on sampling from the input corpora.\todo{writing asynchronous is not sufficient. word2vec already uses asynchronous training}

\item We propose simple and effective approaches to partition and combine submodels preserving word and word-context distributions.

\item we perform extensive experimental evaluation on 14GB of a Wikipedia dump from 2016 to showcase both the scalability and effectiveness of our approaches.
\end{itemize}

%In the next section we provide a more detailed overview of the various techniques employed for improving efficiency of SGNS for large text corpora  and its reliability in case of scarce training data.

==> old-results.tex <==
\begin{figure*} [t] 
	\centering
    \begin{subfigure}[t]{0.47\textwidth}
    	\centering
    	\includegraphics[width=0.7\textwidth]{plots/sample_vs_partition_word.png}
  		\caption{KL-Divergence of word frequency distribution}
        \label{fig:freq}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.47\textwidth}
    	\centering
        \includegraphics[width=0.7\textwidth]{plots/sample_vs_partition_bigram.png}
  		\caption{KL-Divergence of bigram frequency distribution}
    \end{subfigure}
    \caption{plot of sub-corpora size and average KL-Divergence of term frequency distribution}\label{kld}
\end{figure*}



\begin{table}[ht!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cccr}
\hline
model configuration&dimensionality & min-count threshold & vocab. size\\
\hline
\texttt{Baseline}&500,50&100&307,451\\
\texttt{Random (N/10, .)}&500,50&10&187,315\\
\texttt{Partition (N/10, .)}&500,50&10&135,548\\
\texttt{Random (N/100, .)}&500,50&1&165,176\\
\texttt{Partition (N/100, .)}&500,50&1&57,484\\
\hline
\end{tabular}
\label{tab:hyper}
}
\caption{Hyperparameters and statistics of SGNS trained models. $win=10$, $k=5$, $iter=5$}
\end{table}

\begin{table}[ht!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
Approach & Avg. Training Time  &  PCA  & LRA\\
\hline
\texttt{Random(1/100,100)} & 22 mins & 15.16 mins & --* \\
% \hline
\texttt{Partition(1/100,100)} & 19 mins & 15.16 mins & --* \\
% \hline
\texttt{Random(1/10,10)} & 2 Hrs 53 mins & 11.49 mins & 4 Hrs 14 mins \\

\texttt{Partition(1/10,10)} & 2 Hrs 50 mins & 11.49 mins & 4 Hrs 14 mins \\
\hline
\texttt{Baseline} & 36 Hours & -- & -- \\
\hline
\end{tabular}
}
\caption{Wallclock times for training and merging sub-models. Computing LRA on 100 Models timed out after > 10 Hrs}
\label{tab:runtimes}
\end{table}

==> prelim.tex <==
\section{Preliminaries: SGNS}
% \textbf{Notation:} We assume a collection of words $w \in V_W$ and their contexts $c\in V_C$, where $V_W$ and $V_C$ are the word and context vocabularies, the collection of observed word-context pairs as $D$. We use $\#(w, c)$ to denote the number of times the pair $(w, c)$ appears in D. Similarly, $\#(w) = \sum_{c\in V_C} \#(w, c')$ and $\#(c) =  \sum_{w'\in V_W} \#(w', c)$ are the number of times $w$ and $c$ occurred in $D$, respectively. In the embedding produced by SGNS, each word $w \in V_W$ is associated with a vector $\vec{w} \in R^d$ and similarly each context $c \in V_C$ is represented as a vector $\vec{c} \in R^d$. Let $P_D$ denote the empirical bigram distribution (over the word context pairs), i.e., $P_b(w,c) = {\#(w,c)\over |D|}$ and $P_u$ denote the empirical unigram distribution, i.e., $P_u(w) = {\# w\over |D|}$ and $P_u(c)= {\# c\over |D|}$. Let $N$ be the total number of sentences in the original training data. Let $S$ be the set of sentences.

% Note that each word plays the role of the word and a context and therefore the word and context vocabularies are exactly the same. But note that a word will never or seldom appear in its own context and therefore the dot product of word and context vectors for the same word should be zero. Therefore one cannot use the same vector representations for the same word in its two roles. 
% We start with a brief overview of SGNS\@.

% Given a word sequence, $w_1,w_2,\dots,w_{n}$, for training, the skip-gram model seeks to minimize the following objective to learn word embeddings:
% \begin{align*}
% \mathcal{L}_\text{SG}=-\frac{1}{n}\sum_{i=1}^{n}\sum_{\substack{\mid j\mid\leq c\\j\not=0}}\log p(w_{i+j}\mid w_{i}),
% \end{align*}
% where $w_{i}$ is a target word and $w_{i+j}$ is a context word within a window of size $c$. $p(w_{i+j}\mid w_{i})$ represents the probability that $w_{i+j}$ appears within the neighbor of $w_i$, and is defined as

% \begin{align}
% 	p(w_{i+j}\mid w_{i})=\frac{\exp(\tvec{w_i}\cdot\cvec{w_{i+j}})}{\sum_{w\in\vocab}\exp(\tvec{w_i}\cdot\cvec{w})},\label{eq:softmax}
% \end{align}

% where $\tvec{w}$ and $\cvec{w}$ are $w$'s embeddings when it behaves as a target and context, respectively. $\vocab$ represents the vocabulary set.

% Since it is too expensive to optimize the above objective, Mikolov et al.~\cite{mikolov2013linguistic} proposed negative sampling to speed up skip-gram training. This approximates Eq.~(\ref{eq:softmax}) using sigmoid functions and $k$ randomly-sampled words, called \textit{negative samples}. The resulting objective is given as

% \begin{align*}
% 	\mathcal{L}_\text{SGNS}\!=\!-\frac{1}{n}\sum_{i=1}^{n}\sum_{\substack{\mid j\mid\leq c\\j\not=0}}\psi_{w_i,w_{i+j}}^{+}\!+\!k\mathbb{E}_{v\sim q(v)}[\psi_{w_i,v}^{-}],
% \end{align*}

% where $\psi_{w,v}^{+}=\log\sigma(\tvec{w}\cdot\cvec{v})$, $\psi_{w,v}^{-}=\log\sigma(-\tvec{w}\cdot\cvec{v})$, and $\sigma(x)$ is the sigmoid function. The negative sample $v$ is drawn from a smoothed unigram probability distribution referred to as \textit{noise distribution}: $q(v)\propto f(v)^{\alpha}$, where $f(v)$ represents the frequency of a word $v$ in the training data and $\alpha$ is a smoothing parameter ($0<\alpha\leq 1$). 

% The objective is optimized by SGD\@. Given a target-context word pair ($w_{i}$ and $w_{i+j}$) and $k$ negative samples ($v_{1},v_{2},\dots,v_{k}$) drawn from the noise distribution, the gradient of
% $$-\psi_{w_i,w_{i+j}}^{+}-k\mathbb{E}_{v\sim q(v)}[\psi_{w_i,v}^{-}]\approx-\psi_{w_i,w_{i+j}}^{+}-\sum_{k'=1}^{k}\psi_{w_i,v_{k'}}^{-}$$

% is computed. Then, the gradient descent is performed to update $\tvec{w_i}$, $\cvec{w_{i+j}}$, and $\cvec{v_1},\dots,\cvec{v_k}$. SGNS training needs to scan the entire training data multiple times because it has to pre-compute the noise distribution $q(v)$ before performing SGD\@. This makes it difficult to perform incremental model update when additional training data is provided.



==> retrieval_eval.tex <==
\subsection{Evaluation with Retrieval Models}
\label{sec:ret-models}

We further evaluate the asynchronously trained embeddings in a retrieval task. We selected two approaches to utilize embeddings for retrieval. 

\textbf{Neural Translation LM}: We employ a variant of the Neural Translation Language Model~\cite{zuccon2015integrating} to incorporate the trained embeddings. The query likelihood for this retrieval model is computed as follows:

\begin{equation}
P(q|d) = \Pi_{q_i \in q} P_{ntm} (q_i|d)
\end{equation}

\begin{equation}
P_{ntm}(q_i|d) = \Pi_{w \in d} P(q_i|w) P(w|d)
\end{equation}

where w is a unigram found in the document.

\begin{equation}
P(q_i|w) = \frac{\delta(q_i, w)}{\sum_{w' \in V} \delta(w,w')}
\end{equation}

where V is the vocabulary.

Here $\delta$ represents the cosine similarity between the embeddings of the operand unigrams. This value depends on the embeddings used in the retrieval model. For tractability reasons, we restrict $\sum_{w' \in V} \delta(w,w')$ to the neighborhood (n=50) of $w'$.

$P(w|d)$ is computed using a standard maximum likelihood estimator.

\textbf{Query Expansion LM}: In this approach, we use the embeddings to generate query expansions. For each word in the query we select the top 5 closest words (according to cosine distance) as expansion terms. The expanded query is then used to retrieve documents and ranking is performed using query likelihood on unigram language models with dirichlet smoothing ($\mu = 2000$). 

We used the Robust04 TREC test collection (a standard collection for adhoc retrieval tasks) which consists of 250 queries and approximately 500k news articles. All articles were indexed using Lucene with the inbuilt English Analyzer used for tokenization.  

%The test collection used in our experiments is 100 topics (50-150) from the TREC web adhoc retrieval track and the Clueweb09B document collection. Clueweb09B is the english subset of the Clueweb09 collection with over 50 million web pages. We removed all documents with a spam score of 70 or below using the Waterloo spam scorer. The proposed retrieval model was applied to the top 1000 documents (ranked by query likelihood using unigram language models with dirichlet smoothing, $\mu = 2000$ ).

%
% embedding	map@100	p@5	p@10
% base_line.pkl-0.0.run	0.0055	0.0306	0.0316
% partitioning_100_pca.pkl-0.0.run	0.0055	0.0469	0.0418
% partitioning_10_pca.pkl-0.0.run	0.0074	0.049	0.049
% sampling_100_pca_dim_500.pkl-0.0.run	0.0063	0.049	0.0388
% sampling_10_pca_dim_500.pkl-0.0.run	0.0061	0.0367	0.0418
%

% this table will be used for retrieval results
\begin{table}[ht!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
Approach & MAP@100 & P@5 & P@10 \\
\hline
\hline
Neural Translation LM & & & \\
\hline
\texttt{Random(1/100,100)} & 5.28 & 14.54 & 14.94 \\
\texttt{Partition(1/100,100)}& 4.99 & 13.49 & 12.57\\
\texttt{Random(1/10,10)}  & 6.67 & 17.99 & 17.15 \\
\texttt{Partition(1/10,10)} & 6.71 & 18.96 & 17.35 \\
\hline
\texttt{baseline} & 7.22 & 18.23 & 17.55 \\

% \hline
\hline
\hline
%
%base_line.pkl-0.0.run	0.1089	0.2659	0.2361
%partitioning_100_pca.pkl-0.0.run	0.0991	0.2498	0.2261
%partitioning_10_pca.pkl-0.0.run	0.104	0.2627	0.2442
%sampling_100_pca_dim_500.pkl-0.0.run	0.1024	0.2506	0.2245
%sampling_10_pca_dim_500.pkl-0.0.run	0.1041	0.2554	0.2257

\hline
Query Expansion + LM & & & \\
\hline
\texttt{Random(1/100,100)} & 10.24 & 25.06 & 22.45 \\
\texttt{Partition(1/100,100)}& 9.91 & 24.98 & 22.61\\
\texttt{Random(1/10,10)}  & 10.41 & 25.54 & 22.57 \\
\texttt{Partition(1/10,10)} & 10.40 & 26.27 & 24.42 \\
\hline
\texttt{baseline} & 10.89 & 26.59 & 23.61 \\
\hline
\end{tabular}
}
\caption{Retrieval performance measured in terms of MAP, Precision at rank depth 5 and Precision at rank depth 10 for two retrieval methods. Values shown are percentages.}
\label{tab:retperf}
\end{table}

Table~\ref{tab:retperf} shows the effect of using the various embeddings on retrieval performance. Across both approaches we see that the baseline embedding is best performing in all metrics. This can be partly attributed to the larger vocabulary of the baseline embedding model. For the Neural Translation LM, we see that the next best approaches are the partitioning and random sampling approaches of sample size 10. The difference between them is neglible in both MAP and $P@10$. When the sample size is 100, we see that the random sampling approach is significantly better than it's partitioning counterpart in all metrics. $P@10$ is nearly $15\%$ better (0.1494 vs 0.1257) when using random sampling. 

We see a similar trend when using the embeddings to generate query expansions even though the overall differences are smaller. Our results seem to indicate that asynchronous training for embeddings, while not better, are competitive compared to the baseline when it comes to adhoc retrieval tasks.  

==> theory.tex <==
\section{Theoretical Analysis}
We support the the choice of \random  division strategy by showing that the corresponding unigram and bigram distributions are indeed preserved in the samples. We first show that the expected frequency of a word in any sub-corpus sampled using \random is equal to its probability of occurrence in the original corpus. 
%Using Chebyshev inequality we then bound its deviation from the expected value. 

Let $|\w|_C$ denote the frequency of word $\w$ in a given corpus $C$. Let $P_C(\w)$ be the probability that a randomly drawn out word from $C$ is the word $\w$. Note that the empirical probability of drawing out word $\w$ is equal to the number of occurrences of $\w$ in $C$ divided by the total number of words in $C$.
%Then $\Pr(|\w|_C>0)$ is the probability that the word $\w$ occurs at least once in the corpus $C$. Note that $\Pr(|\w|_C>0)$ is simply the probability distribution of $\w$ in $C$. Let $\mathcal{T}_C$ denote the total word count in corpus $C$. For notational convenience we denote $\Pr(|\w|_C>0)$ by $P_C(\w)$. 
We prove the following theorem.
\begin{theorem}
For any sub-corpus $C'$ drawn from the original corpus $C$ using \random and any word , $\w$ we have 
$$\E\left( |\w|_{C'} \over \mathcal{T}_{C'} \right) = P_C(w)$$.
\end{theorem}
\begin{proof}
First we model the probability of the sub-corpus $C'$. Let $x$ and $y$ be random variables  such that the frequency of a word $|\w|_{C'} =x$ and $\mathcal{T}_{C'}=y$. Let the total number of sentences in $C$ be $N$ and in $C'$ be $uN$. Then the probability of the corpus $C'$ with $x$ occurrences of word $\w$ and $y$ being the total word count is given by
\begin{align*}
&\Pr(C'| |C'|=uN,|\w|_{C'} =x, \mathcal{T}_{C'}=y ) \\ 
& = u^{uN} \Pr(\mathcal{T}_{C'}=y) {y \choose x} (P_C(w))^x (1-P_C(w))^{y-x}, 
\end{align*}
where the first term $u^{un}$ is the probability of drawing out $uN$ sentences of sub-corpora  $C'$ from $C$. Now
\begin{align*}
\E\left( x\over y \right) = & \sum_{x,y} { x \over y } \Pr(C'| |C'|=uN,|\w|_{C'} =x, \mathcal{T}_{C'}=y ) \\
=& \sum_{x,y} { x \over y } {y \choose x} (P_C(w))^x (1-P_C(w))^{y-x}  u^{uN} \Pr(\mathcal{T}_{C'}=y)\\
=& \sum_{x,y} { (y-x+1) \over y  } {y \choose x -1} (P_C(w))^{x-1} (1-P_C(w))^{y-x}\\
& \cdot u^{uN} \Pr(\mathcal{T}_{C'}=y)\\
=&{ P_C(w) \over 1-P_C(w) }  \cdot \bigg( \sum_{x,y}  {y \choose x -1}(P_C(w))^{x-1} (1-P_C(w))^{y-x+1}  \\
& \cdot  u^{uN} \Pr(\mathcal{T}_{C'}=y) + \\
&\sum_{x,y} { x-1 \over y  } {y \choose x -1} (P_C(w))^{x-1} (1-P_C(w))^{y-x+1} \\
& \cdot u^{uN} \Pr(\mathcal{T}_{C'}=y) \bigg) \\
= &{ P_C(w) \over 1-P_C(w) }  \left(1+ \E\left({x \over y}\right) \right) \\
&\Rightarrow \E\left( x\over y \right) = P_C(w)
\end{align*}
\end{proof}

We now prove that as long as $P_C(\w)$ obeys a certain condition, with high probability the word $\w$ exists in at least one sub-corpora. We assume that the word count in each sentence is equal to some constant $\ell$.
\begin{theorem}
Let $u=r/100$ where $r$ is the sampling rate. If
\begin{equation}\label{eq:pw} P_C(w)> 1-(1-u)^{1-u \over \ell u}, \end{equation}
then the expected number of randomly sampled sub-corpora with a missing word $\w$ is equal to $\exp(-O(N))$.
% $$\Pr(\text{word $\w$ is missing in all samples}) {\xrightarrow{N\rightarrow \infty } }0 .$$
\end{theorem}
\begin{proof}
We will show that for arbitrary word $\w$ if $P_C(w)$ obeys Equation~\eqref{eq:pw} the expected number of sub-corpora (sampled using \random from any given corpus) is exponential small in size of the original Corpus $N$. Let $X$ be the random variable denoting the total number of sub-corpora of size $uN$ in which the word $\w$ is missing.
$$\E(X) = {N \choose uN} u^{\ell uN}   (1-P_C(w))^{\ell uN}.$$
Using Stirling's approximation,
$\sqrt{2\pi x} \left( {x\over e}\right)^x \le x! \le e\sqrt{2\pi x} \left( {x\over e}\right)^x $ we obtain 
$${N \choose uN}\le u^{-uN}\cdot(1-u)^{-(1-u)N} \cdot {\exp(1)\over  \sqrt{2\pi N u(1-u)}}. $$
Denoting $-u \log u -(1-u) \log u$ by $H(u)$ we obtain
\begin{align*}
\E(X)\le &\sum_y \exp(NH(u)) \cdot u^{uN} (1-P_C(w))^{\ell uN} \\
&\le  \exp(NH(u)) \cdot u^{uN}  ((1-P_C(w))^{ \ell un}) \\
& = \exp(O(N (H(u) + u \log u + u \ell \log (1-P_C(w))))
\end{align*}
Now $\E(X)= e^{-O(N)}$ if 
\begin{align*}
& H(u) + u \log u +  u \ell \log (1-P_C(w)) < 0 \\
 & \Rightarrow -(1-u)\log(1-u) + u \ell \log (1-P_C(w)) < 0 \\
 & \Rightarrow 1-P_C(w) < (1-u)^{1-u\over \ell u},
\end{align*}
which implies Equation \eqref{eq:pw}.

% Using Markov's Inequality we have
% $$ \Pr(X\ge 1)\le \E(X) = e^{-O(N)},$$
% thereby completing the proof.
\end{proof}
% \begin{theorem}
% Let $u=r/100$ where $r$ is the sampling rate. If
% \begin{equation}\label{eq:pw} P_C(w)> 1-(1-u)^{1-u \over \ell u}, \end{equation}
% then 
% $$\Pr(\text{word $\w$ is missing in all samples}) {\xrightarrow{N\rightarrow \infty } }0 .$$
% \end{theorem}
% \begin{proof}
% We will show that for arbitrary word $\w$ if $P_C(w)$ obeys Equation~\eqref{eq:pw} the expected number of sub-corpora (sampled using \random from any given corpus) is exponential small in size of the original Corpus $N$. Let $X$ be the random variable denoting the total number of sub-corpora of size $uN$ such that a word $\w$ is missing from all of these corpora.
% $$\E(X) = {N \choose uN} u^{\ell uN}   (1-P_C(w))^{\ell uN}.$$
% Using Stirling's approximation,
% $\sqrt{2\pi x} \left( {x\over e}\right)^x \le x! \le e\sqrt{2\pi x} \left( {x\over e}\right)^x $ we obtain 
% $${N \choose uN}\le u^{-uN}\cdot(1-u)^{-(1-u)N} \cdot {\exp(1)\over  \sqrt{2\pi N u(1-u)}}. $$
% Denoting $-u \log u -(1-u) \log u$ by $H(u)$ we obtain
% \begin{align*}
% \E(X)\le &\sum_y \exp(NH(u)) \cdot u^{uN} (1-P_C(w))^{\ell uN} \\
% &\le  \exp(NH(u)) \cdot u^{uN}  ((1-P_C(w))^{ \ell un}) \\
% & = \exp(O(N (H(u) + u \log u + u \ell \log (1-P_C(w))))
% \end{align*}
% Now $\E(X)= e^{-O(N)}$ if 
% \begin{align*}
% & H(u) + u \log u +  u \ell \log (1-P_C(w)) < 0 \\
%  & \Rightarrow -(1-u)\log(1-u) + u \ell \log (1-P_C(w)) < 0 \\
%  & \Rightarrow 1-P_C(w) < (1-u)^{1-u\over \ell u},
% \end{align*}
% which implies Equation \eqref{eq:pw}.

% Using Markov's Inequality we have
% $$ \Pr(X\ge 1)\le \E(X) = e^{-O(N)},$$
% thereby completing the proof.
% \end{proof}

\section{Extra Experimental Setup Details}
The statistics concerning the \random, \partition and \shuffle approaches and the \baseline model are presented in Table~\ref{tab:hyper}. 
% The models have an associated sampling rate  of $r\%$ associated (i.e. $10\%$), this refers to the data being split into $10$ parts and the actual model being composed of 10 sub-models of size $N/10$ each, where $N$ is the total number of sentences. The hyper-parameters and statistics concerning the \random, \partition and \shuffle approaches and the baseline model are presented in Table~\ref{tab:hyper}.
\begin{table}[ht!]
\footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
Model&Sampling& Min-count  & Vocab. size\\
%& vocab. size \\
&rate& threshold & (common)\\
% & (union)\\
\hline
%\texttt{Baseline}&--&100&307,451\\
\baseline &--&100&300,000\\
\random &10\%&10&187,315\\
\partition &10\%&10&135,548\\
\shuffle &10\%&--&299,790\\
\random &1\%&1&60,848\\
\partition &1\%&1&47,692\\
\shuffle &1\%&--&262,390\\
\hline
\end{tabular}
}
\caption{Statistics of SGNS trained models. The windows size is 10, dimension of each model is 500, count of negative samples is 5, number of iteration is 5 and the all the models or sub-models are calculated using 10 threads.}
\label{tab:hyper}
\end{table}


\begin{figure*}[h!]	
\centering

    \begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/AP.pdf}
    \end{subfigure}
    \begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/Battig.pdf}
    \end{subfigure}
    \begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/RG65.pdf}
    \end{subfigure}
	\begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/RW.pdf}
	\end{subfigure}
    \begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/Google.pdf}
    \end{subfigure}
    \begin{subfigure}{.30\linewidth}
  		\includegraphics[width=\linewidth]{n-by-10-alr-shuffle-pdfs/SemEval2012_2.pdf}
    \end{subfigure}

	\caption{Box Plots showing the effectiveness of merging Sub-Models with the \texttt{Shuffle + \problem} approach. \problem initialized with PCA (Epochs = $3$, Sample Rate = $10\%$, Dimensions = $500$). The red line indicates the \baseline   performance. Top and bottom of the boxes represent one quartile above and below the mean. The whiskers on top of and under the boxes represent the highest and the lowest values that are within the 1.5 IQR (interquartile range) of the upper and lower quartile. Dots are outliers that are even higher or lower than the ends of whiskers.}
	\label{fig:n-10-box}
\end{figure*}

While merging using \pca, we used the TruncatedSVD implementation provided in scikit-learn~\footnote{http://scikit-learn.org}. For the matrix transformations in \problem we used the orthogonal\_procrustes method provided in SciPy (scipy.linalg.orthogonal\_procrustes). Both of these Python modules support BLAS acceleration. Note that using orthogonal Procrustes is considerably slower since SVD is performed multiple times as opposed to once for PCA. Additionally, \problem is run for multiple epochs.

\begin{figure*}[ht!]
	\centering
	
    \begin{subfigure}{.24\linewidth}
    	\centering
  		\includegraphics[width=\linewidth]{sampling_plots/AP.eps}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    	\centering
  		\includegraphics[width=\linewidth]{sampling_plots/Battig.eps}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
        \centering
  		\includegraphics[width=\linewidth]{sampling_plots/MEN.eps}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    	\centering
  		\includegraphics[width=\linewidth]{sampling_plots/RG65.eps}
    \end{subfigure}
	\begin{subfigure}{.24\linewidth}
    	\centering
  		\includegraphics[width=\linewidth]{sampling_plots/RW.eps}
	\end{subfigure}
    \begin{subfigure}{.24\linewidth}
   		\centering
   		\includegraphics[width=\linewidth]{sampling_plots/WS353.eps}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
    	\centering
  		\includegraphics[width=\linewidth]{sampling_plots/Google.eps}
    \end{subfigure}
    \begin{subfigure}{.24\linewidth}
	    \centering
  		\includegraphics[width=\linewidth]{sampling_plots/SemEval.eps}
    \end{subfigure}
    \caption{Comparison of different sampling rates on the Wikipedia data set. Merged using \problem. Sampled using \shuffle.}
	\label{fig:sampling-comparison}
\end{figure*}

\section{Effect of Sampling Rate and Sub-Model Counts}
\label{sec:sample-sizes-counts}
In this section, we first discuss results from an experiment where we vary the sampling rate $r$ while fixing the merging strategy (\problem) and sampling strategy (\shuffle). Then we discuss the results when varying only the number of sub-models being merged given a fixed sampling rate ($r$=10\%).

Figure~\ref{fig:sampling-comparison} illustrates the performance of our trained representations in various benchmarks for increasing sampling rates. We find two distinct trends here. 
For \ws, \google and \semeval, increased sampling rate (fewer sub-models) leads to better performance. This shows that increased parallelization does not always translate to good performance particularly in the analogy task which is considered to be a difficult task. Merging fewer sub-models that have encountered more training data is beneficial for these benchmarks. 

In the remaining 5/8 benchmarks, we find that lower sampling rates yield good results. 5-10\% sampling rate for our configuration gives the best results. With a lower sampling rate, training sub-models is considerably faster. Merging these models leads to good performance as well, with \baseline being bettered in all benchmarks except \men.  

Now we discuss the effect of merging a varying number of sub-models. Figure~\ref{fig:n-10-box} shows the relationship between count of merged sub-models and performance in each benchmark. We fix the $r$ as 10\% leading to a maximum of 10 sub-models. 

Immediately we can notice a steady increase in performance (in most benchmarks) as the number of sub-models merged increases. Benchmarks with more unique words benefit the most from merging more sub-models (see \ap vs \rw in Figure~\ref{fig:n-10-box}). When we select just a single model out of 10 (\#(sub-models) = 1), performance usually tends to be below the \baseline. This is especially true for \google and \battig where even the best model is worse than \baseline. 
Next we observe the plateauing of performance when merging more models. When utilizing a smaller sampling rate, this observation indicates that we can be more selective when merging. Instead of merging 100 sub-models produced when $r$=0.1\%, we can select a smaller number of sub-models on which to perform \problem. This is useful to speed up the overall training time since merging a large number of models using \problem is slow. This point is discussed in further detail in Section~\ref{sec:scaling}.

The performance also varies depending on the task at hand. We notice that for certain tasks/benchmarks merging new sub-models does not monotonically improve performance. For \rg, merging more than 3 sub-models is detrimental. For \semeval merging more than 5 decreases performance and similarly for \battig, 6 sub-models give best performance. 

These results show that merging more sub-models leads to improved performance over \baseline but for optimal performance in certain tasks we must carefully choose the number of sub-models to merge. 



